Retinopathy of Prematurity Stage Diagnosis Using Object Segmentation and Convolutional Neural Networks

Retinopathy of Prematurity (ROP) is an eye disorder primarily affecting premature infants with lower weights. It causes proliferation of vessels in the retina and could result in vision loss and, eventually, retinal detachment, leading to blindness. While human experts can easily identify severe stages of ROP, the diagnosis of earlier stages, which are the most relevant to determining treatment choice, are much more affected by variability in subjective interpretations of human experts. In recent years, there has been a significant effort to automate the diagnosis using deep learning. This paper builds upon the success of previous models and develops a novel architecture, which combines object segmentation and convolutional neural networks (CNN) to construct an effective classifier of ROP stages 1-3 based on neonatal retinal images. Motivated by the fact that the formation and shape of a demarcation line in the retina is the distinguishing feature between earlier ROP stages, our proposed system first trains an object segmentation model to identify the demarcation line at a pixel level and adds the resulting mask as an additional "color" channel in the original image. Then, the system trains a CNN classifier based on the processed images to leverage information from both the original image and the mask, which helps direct the model's attention to the demarcation line. In a number of careful experiments comparing its performance to previous object segmentation systems and CNN-only systems trained on our dataset, our novel architecture significantly outperforms previous systems in accuracy, demonstrating the effectiveness of our proposed pipeline.

==> acknowledgment.tex <==
\section*{Acknowledgement}
The research of this paper is conducted under the close mentorship of Prof. Benyuan Liu at the University of Massachusetts Lowell. I thank the members of his graduate lab group for their stimulating discussion and help along the way. Without them or Prof. Liu, none of this work would have been possible. 

==> tables/binary-oo-values.tex <==
mean, std
(0.05760112502080307, 0.03454983612873903)

==> tables/perfect-oo-classifier.tex <==
[[153 151  36]
 [ 33 290  73]
 [  2 144 208]]
              precision    recall  f1-score   support

     Stage 1       0.81      0.45      0.58       340
     Stage 2       0.50      0.73      0.59       396
     Stage 3       0.66      0.59      0.62       354

    accuracy                           0.60      1090
   macro avg       0.66      0.59      0.60      1090
weighted avg       0.65      0.60      0.60      1090

